Isoperimetric inequalities for wave fronts and a generalization of Menzin's conjecture for bicycle monodromy on surfaces of constant curvature

We prove generalizations of the isoperimetric inequality for both spherical and hyperbolic wave fronts (i.e. piecewise smooth curves which may have cusps). We then discuss "bicycle curves" using the generalized isoperimetric inequalities. The euclidean model of a bicycle is a unit segment AB that can move so that it remains tangent to the trajectory of point A (the rear wheel is fixed on the bicycle frame). We extend this definition to a general Riemannian manifold, and concern ourselves in particular with bicycle curves in the hyperbolic plane H^2 and on the sphere S^2. We prove results along the lines of those proven by Levi and Tabachnikov and resolve both spherical and hyperbolic versions of Menzin's conjecture, which relates the area bounded by a curve to its associated monodromy map.

==> sphericalarclength.tex <==
	\begin{theorem}[$S^2$]
		\begin{equation}\label{spharclength}
			\dfrac{ds}{dt} = \sqrt{\sin^2 (l) k^2 +1}.
		\end{equation}
		
	\end{theorem}
	\begin{proof}
		 Parameterize $\gamma$ by $t$. We have that \[ \Gamma = \gamma \cos(l) + \gamma' \sin(l) \] and therefore
		\[\Gamma ' = \gamma' \cos(l) + \gamma'' \sin(l).\]
		 From $\gamma' \cdot \gamma' = 1$, we get $\gamma' \cdot \gamma '' = 0$, so
		\begin{eqnarray*}
			 &\Gamma ' \cdot \Gamma' &= 2\gamma' \cdot \gamma '' \cos(l)\sin(l) + \gamma' \cdot \gamma ' \cos^2(l) + \gamma '' \cdot \gamma '' \sin^2(l) \\
			& &= \cos^2(l) + \gamma'' \cdot \gamma'' \sin^2(l)
		\end{eqnarray*}
		From $\gamma \cdot \gamma = 1,$ we have $\gamma \cdot \gamma' = 0,$ and therefore $\gamma '' \cdot \gamma = - \gamma' \cdot \gamma' = -1$. We can then decompose $\gamma ''$ into radial and tangential components:
		\[ \gamma '' = (\gamma''\cdot \gamma)\gamma + \gamma''_g = -\gamma + \gamma''_g  \]
		We then have 
		\[ \gamma '' \cdot \gamma'' = \gamma \cdot \gamma + k^2 = 1 + k^2 \]
		and so the previous expression becomes
		\begin{eqnarray*}
			&\Gamma ' \cdot \Gamma' &= \cos^2 (l) + (1 + k^2)\sin^2 (l) \\
			& &= \sin^2 (l) k + 1
		\end{eqnarray*}
		which implies that $\dfrac{ds}{dt} = \sqrt{\sin^2(l) k + 1}.$
	\end{proof}
